Hard-constrained Physics-informed Neural Networks for Interface Problems

Physics-informed neural networks (PINNs) have emerged as a flexible framework for solving partial differential equations, but interface problems remain challenging because continuity and flux conditions are typically imposed through soft penalty terms, leading to imperfect interface enforcement and degraded accuracy near interfaces. We introduce two ansatz-based hard-constrained PINN formulations for interface problems that embed the interface physics into the solution representation, decoupling interface enforcement from PDE residual minimization. The windowing approach constructs the trial space from compactly supported windowed subnetworks so that interface continuity and flux balance are satisfied by design. The buffer approach discretely hard-constrains subnetworks with additive buffer functions that enforce boundary and interface constraints at sampled points through a lightweight correction. We study both formulations on one- and two-dimensional elliptic interface benchmarks against soft-constrained baselines. A statistical study in one dimension shows that the windowing approach occasionally attains very high accuracy (as low as $O(10^{-9})$) on simple structured cases, but its rigid ansatz makes training stiff, so its median errors are often worse than the baselines. In contrast, the buffer approach achieves the smallest median error (as low as $O(10^{-5})$) across a wider range of source terms and interface configurations. In two dimensions, the buffer formulation is more robust for general geometries, while the windowing construction is more sensitive to overlap and corner effects and over-constrains the problem. These results position the buffer method as a straightforward and promising approach for interface problems, with the search for an optimal buffer function form left for future work.

==> Makefile <==
.PHONY: all DIFF RESPONSE clean diffclean responseclean realclean

LATEX = pdflatex
TALKNAME = manuscript
CHAPTERS = $(wildcard sections_*.tex)
FIGURES = $(wildcard figures_*.tex)
DIFFFILES = $(CHAPTERS:sections_%.tex=sections-diff_%.tex)
REFS = references

SOURCEFILES = $(TALKNAME).tex packages.tex notations.tex $(REFS).bib

all: $(TALKNAME).pdf

DIFF: diff.pdf

RESPONSE: response.pdf summary_rev.pdf

$(TALKNAME).pdf: $(TALKNAME).tex packages.tex notations.tex $(REFS).bib $(FIGURES) $(CHAPTERS)
	$(LATEX) $(TALKNAME)
	bibtex $(TALKNAME)
	$(LATEX) $(TALKNAME)
	$(LATEX) $(TALKNAME)

# --math-markup=off: comment out deleted equations entirely rather than
# interleaving \DIFdel fragments inside math, which renders as a mangled
# struck-out equation.  Prose markup, including inline math, is unaffected.
LATEXDIFFFLAGS = -t CFONT --math-markup=off

sections-diff_%.tex: sections_%.tex sections-orig_%.tex
	latexdiff $(LATEXDIFFFLAGS) sections-orig_$*.tex sections_$*.tex > $@

diff.pdf: diff.tex packages.tex notations.tex $(REFS).bib $(FIGURES) $(DIFFFILES)
	$(LATEX) diff
	bibtex diff
	$(LATEX) diff
	$(LATEX) diff

response.pdf: response.tex packages.tex notations.tex
	$(LATEX) response
	$(LATEX) response

summary_rev.pdf: summary_rev.tex packages.tex notations.tex
	$(LATEX) summary_rev
	$(LATEX) summary_rev

clean:
	rm -f *.vrb *.tex~ *.toc *.aux *.log *.nav *.out *.snm *.flc *.gz *.bbl *.blg *.md5 *.auxlock *.cb *.cb2 *.fdb_latexmk *.fls *.dpth *.spl

diffclean:
	rm -f diff.pdf $(DIFFFILES)

responseclean:
	rm -f response.pdf summary_rev.pdf

realclean: clean diffclean responseclean
	rm -f $(TALKNAME).pdf


==> packages.tex <==
\usepackage{amssymb, amsmath}
\usepackage{stmaryrd}

\usepackage{hyperref}

\usepackage{comment}
\usepackage{arydshln}
\usepackage{bm}
\usepackage[textsize=tiny,
disable
]{todonotes}
\usepackage{multirow}

\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{tikz}
\usetikzlibrary{positioning}
% \usepackage{pgfplotstable}
\usepackage{pgfplots}
\pgfplotsset{compat=1.10}
\usepgfplotslibrary{groupplots,fillbetween}
\usetikzlibrary{spy, backgrounds}
\usetikzlibrary{shapes.geometric, arrows.meta}

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFaddtex}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdeltex}[1]{{\protect\color{red}\sout{#1}}} %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
\providecommand{\DIFmodbegin}{} %DIF PREAMBLE
\providecommand{\DIFmodend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
%% Inside floats latexdiff comments out the tabular scaffolding but keeps the
%% \DIF*FL fragments, which ulem's \sout/\uwave cannot span.  Additions in
%% tables and captions are marked with colour only (no underline); deletions
%% are dropped entirely, since a struck-out copy of an old table or caption
%% is unreadable next to the new one. %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{{\protect\color{blue}#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF HYPERREF PREAMBLE %DIF PREAMBLE
\providecommand{\DIFadd}[1]{\texorpdfstring{\DIFaddtex{#1}}{#1}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{\texorpdfstring{\DIFdeltex{#1}}{}} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF

==> sections_target_physics.tex <==
\section{Model problems}
We consider a generic spatial domain composed of multiple disjoint subdomains,
\begin{equation}
\Omega = \bigcup_m^M \Omega_m,
\end{equation}
where each subdomain $\Omega_m$ has distinct physical properties. We denote the subdomain boundary of $\Omega_b$ as $\Gamma_b=\partial\Omega_b\cap\partial\Omega$,
and the interface between $\Omega_i$ and $\Omega_j$ as $\Gamma_{ij} = \partial\Omega_i\cap\partial\Omega_j$.
Throughout this work, the following Poisson equation serves as a representative problem to illustrate the proposed methods
\begin{equation}\label{eq:poisson}
\LHS[u] \equiv -\nabla\cdot\kappa(\bx)\nabla u(\bx) = f(\bx)
\qquad
\forall\bx\in\Omega,
\end{equation}
where the diffusivity $\kappa(\bx)$ has discontinuities
at the subdomain interfaces.
For the interface $\Gamma_{ij}$,
the physics state $u(\bx)$ and its flux are continuous across the interfaces,
\begin{subequations}\label{eq:itf_cond}
\begin{equation}
\jump{u}_{ij} \equiv u\big|_{\Omega_i} - u\big|_{\Omega_j} = 0
\qquad
\forall\bx\in\Gamma_{ij}
\end{equation}
\begin{equation}
\avg{\bn\cdot\kappa\nabla u}_{ij}
\equiv \frac{\bn\cdot\kappa\nabla u\big|_{\Omega_i} + \bn\cdot\kappa\nabla u\big|_{\Omega_j}}{2}
= 0,
\qquad
\forall\bx\in\Gamma_{ij},
\end{equation}
\end{subequations}
where $\bn$ is the outward-facing normal vector of each subdomain. We consider three one-dimensional Poisson problems with analytic solutions to evaluate the approximation accuracy. In addition, we also consider a two-dimensional problem with three distinct spatially varying source terms.
\par
Throughout this study, hard-constrained PINN models are trained against the residual loss
for the physics governing equation,
\begin{equation}\label{eq:J-int}
\cJ_{physics} = \sum_{k}^K ( -\nabla\cdot\kappa(\bx_k)\nabla u(\bx_k) - f(\bx_k) )^2,
\end{equation}
where $\{\bx_k\}_{k=1}^K\subset\Omega$ are collocation points. For soft-constrained methods, residual losses from boundary and interface conditions are computed in addition to the physics loss:
\begin{equation}\label{eq:J-dbc_1}
\cJ_{dbc} = \sum_{k}^{K_d}( u(x_k) - g_d(x_k) )^2,
\end{equation}
\begin{equation}\label{eq:J-dbc_2}
\cJ_{nbc} = \sum_{k}^{K_n} ( \bn\cdot \nabla u(x_k) - g_n(x_k) )^2,
\end{equation}
\begin{equation}\label{eq:J-dbc_3}
\cJ_{int} = \sum_{k}^{K_i} ( u(x_k)\big|_{\Omega_i}  - u(x_k)\big|_{\Omega_j}  )^2,
\end{equation}
\begin{equation}\label{eq:J-dbc_4}
\cJ_{fint} = \sum_{k}^{K_i} ( \bn\cdot \kappa \nabla u(x_k)\big|_{\Omega_i} - \bn\cdot \kappa \nabla u(x_k)\big|_{\Omega_j} )^2,
\end{equation}

To demonstrate the efficacy of the proposed methods, we present a sequence of example problems selected to exhibit progressively increasing levels of difficulty.
% \todo[inline]{Sumanta, can you describe the loss for soft-constraining approaches?}
\todo[inline]{Kevin: move the model problems below $\downarrow$ after the method section.}

\subsection{Problem 1: Uniform source term with single interface}\label{subsec:1interface}
First, we solve the one-dimensional diffusion equation on a composite domain consisting of two materials characterized by different diffusivities. We consider the one-dimensional domain $\Omega=[0,1]$
composed of two subdomains with their interface at $\Gamma_{12} = \{x_{itf}\equiv 0.5\}$.
The diffusivity $\kappa$ is piece-wise constant,
\begin{equation}
\kappa =
\begin{cases}
\kappa_1 \equiv 0.1 & x < x_{itf} \\
\kappa_2 \equiv 1 & x \ge x_{itf},
\end{cases}
\end{equation}
and the source term $f(\bx)=1$ is constant over the domain.
We consider homogeneous Dirichlet boundary conditions at the left and right boundaries,
\begin{equation}\label{eq:homo-diri-bc}
u(0) = u(1) = 0.
\end{equation}
This problem has an analytic solution of the form,
\begin{equation}
u(\bx) =
\begin{cases}
-\frac{x^2}{2\kappa_1} + c_1\frac{x}{\kappa_1} + c_2 & x < x_{itf} \\    
-\frac{x^2}{2\kappa_2} + c_3\frac{x}{\kappa_2} + c_4 & x \ge x_{itf}.
\end{cases}
\end{equation}
The coefficients $c_1$, $c_2$, $c_3$ and $c_4$ are determined
by the boundary and interface conditions,
which constitutes the following system,
\begin{equation}
\begin{pmatrix}
0 & 1 & 0 & 0 \\
0 & 0 & \frac{1}{\kappa_2} & 1 \\
\frac{x_{itf}}{\kappa_1} & 1 & -\frac{x_{itf}}{\kappa_2} & -1 \\
x_{itf} & 0 & -x_{itf} & 0
\end{pmatrix}
\begin{pmatrix}
c_1 \\ c_2 \\ c_3 \\ c_4
\end{pmatrix}
=
\begin{pmatrix}
0 \\ \frac{1}{2\kappa_2} \\ \frac{x_{itf}^2}{2\kappa_1} - \frac{x_{itf}^2}{2\kappa_2} \\ 0
\end{pmatrix}.
\end{equation}

\subsection{Problem 2: Uniform source term with three interfaces}\label{subsec:3interface}
We solve the one-dimensional diffusion equation on a domain with three interfaces. The interfaces are located at $\Gamma=\{0.25, 0.5, 0.75\}$~\cite{sarma2024interface},
with the same source term $f(\bx)=1$ and the same boundary condition (\ref{eq:homo-diri-bc}) as the first problem.
The analytical solution can be found in~\ref{app:prob2-sol}~and~\cite{sarma2024interface}.

\subsection{Problem 3: Spatially varying source term with one interface}\label{subsec:1int-spatially-varying}
We consider the one-dimensional diffusion equation with a spatially varying source term across the interface. The interface is located at $\Gamma=\{x_{itf}=0.5\}$, and the source term is defined as,
\begin{equation}
-\nabla\cdot(\kappa\nabla u)
=
\begin{cases}
f_0 & x < x_{itf}\\
f(x) \equiv a\exp\left(-\frac{(x-x_c)^2}{w^2}\right) & x > x_{itf},
\end{cases}
\end{equation}
with $f_0=-0.05$, $a=1$, $x_c=0.75$, and $w=0.1$.
For the boundary condition, we consider a homogeneous Neumann condition at $x=0$ and a homogeneous Dirichlet condition at $x=1$,
\begin{subequations}
\begin{equation}
\Dpartial{u}{x}(0) = 0
\end{equation}
\begin{equation}
u(1) = 0.
\end{equation}
\end{subequations}
This problem has an analytic solution of the form,
\begin{equation}
u(\bx) =
\begin{cases}
-f_0\frac{x^2}{2\kappa_1} + c_1\frac{x}{\kappa_1} + c_2 & x < x_{itf} \\
F(x) + c_3\frac{x}{\kappa_2} + c_4 & x \ge x_{itf},
\end{cases}
\end{equation}
where $F(x)$ is the double integral of $f(x)$,
\begin{equation}
F(x) = \frac{aw\sqrt{\pi}}{2\kappa_2}(x - x_c)\,\mathrm{erf}\!\left(\frac{x-x_c}{w}\right)
+ \frac{aw^2}{2\kappa_2}\exp\left(-\frac{(x-x_c)^2}{w^2}\right).
\end{equation}
The coefficients are determined by the following system that describes the boundary and interface conditions,
\begin{equation}
\begin{pmatrix}
1 & 0 & 0 & 0 \\
0 & 0 & \frac{1}{\kappa_2} & 1 \\
\frac{x_{itf}}{\kappa_1} & 1 & -\frac{x_{itf}}{\kappa_2} & -1 \\
1 & 0 & -1 & 0
\end{pmatrix}
\begin{pmatrix}
c_1 \\ c_2 \\ c_3 \\ c_4
\end{pmatrix}
=
\begin{pmatrix}
0 \\ F(1) \\ \frac{f_0x_{itf}^2}{2\kappa_1} - F(x_{itf}) \\ f_0x_{itf} - F_x(x_{itf})
\end{pmatrix},
\end{equation}
where $F_x(x)$ is the integral of $f(x)$,
\begin{equation}
F_x(x) = \frac{aw\sqrt{\pi}}{2\kappa_2}\,\mathrm{erf}\!\left(\frac{x-x_c}{w}\right).
\end{equation}

\subsection{Problem 4: Slanted interface in a two-dimensional domain}\label{subsec:2dpoisson}
Finally, we consider a two-dimensional rectangular domain with a slanted interface.
The domain is defined on $\bx = (x, y) \in \Omega=[0, 2]\times[0, 1]$.
The interface is defined as $\Gamma = \{(x, y) | y = (x - x_b) / (x_t - x_b) \}$ with $x_b=0.8$ and $x_t=1.2$.
The diffusivity is defined as
\begin{equation}
\kappa
=
\begin{cases}
0.1 & y >\frac{x - x_b}{x_t - x_b} \\
1 & \text{otherwise}.
\end{cases}
\end{equation}
A homogeneous Dirichlet condition is assigned on the right-side subdomain boundary,
\begin{equation}
u(\bx)=0 \qquad\text{on }\partial\Omega_R,
\end{equation}
with
$\partial\Omega_R=\{(x,y)| y < (x - x_b) / (x_t - x_b)\} \cap \{(x, y)|y=0 \text{ or } 1\text{, or } x=2\}$.
On the left-side subdomain, a
homogeneous Neumann condition is assigned,
\begin{equation}
\bn\cdot\kappa\nabla u(\bx)=0 \qquad\text{on }\partial\Omega_L,
\end{equation}
with
$\partial\Omega_L=\{(x,y)| y > (x - x_b) / (x_t - x_b)\} \cap \{(x, y)|y=0 \text{ or } 1\text{, or } x=0\}$.
The source term is defined as the sum of
three Gaussian sources,
\begin{equation}\label{eq:2dpoisson-f}
f(\bx)
=
\sum_{i=1}^3
A_i\exp\left( - \frac{\Vert \bx - \bx_i \Vert^2}{r_i^2} \right),
\end{equation}
with $\{\bx_i\} = \{(0.3, 0.6), (1, 0.2), (1.6, 0.7)\}$,
$\{r_i\} = \{0.08, 0.2, 0.1\}$
and
$\{A_i\} = \{10, 20, 15\}$.
\begin{figure}[tbph]
\hspace*{-1.8cm}
    \input{figures_2dpoisson_truth.tex}
    \caption{Model problem with a slanted interface in a two-dimensional domain: (a) solution; and (b) source term.}
    \label{fig:2dpoisson_truth}
\end{figure}
Figure~\ref{fig:2dpoisson_truth} shows the solution and source term of the model problem.
The solution is obtained via a finite-element solver~\cite{mfem}
with a fine mesh of $\sim132,000$ grid points.
